Neighbourhood semantics and axioms for strategic fragment of classical stit logic

STIT (sees to it that) semantics is one of the most prominent tools in modal logic of agency, widely used among both philosophers and responsible AI scholars. STIT logic surveys the properties of agents seeing to it that some state of affairs holds without specifying concrete actions by which that state of affairs is guaranteed. In comparison with other multi-agent modal logics, the main advantage of STIT theories is expressive power. STIT logic allows to study not only statements about agents abilities to perform certain actions (as it is in variations of Coalition Logic or Propositional Dynamic Logic), but about what choices they make and what they de-facto achieve as well. Nevertheless, in some occasions such expressivity may be redundant. This paper surveys a specific fragment of classical STIT logic, which has only strategic modal operator, standing for the fact that agent has an ability to see to it that some state of affairs holds. The neighbourhood semantics for the fragment is presented, accompanied with the soundness, canoniciy hence strong completeness results. Furthermore, the paper presents basic considerations on epistemic extension of the presented fragment.

==> extension.tex <==
\subsection{Epistemic extension with action types}

It was proposed to extend both language and model in order to formalize epistemic aspects of ability. To be more precise, authors argue that agents always certain about action \textit{type} they execute, but they may be unaware about which action \textit{token} will be the result of that execution. For example, if an agent tries to open a door with a key, but she is unaware if the key is the right one, she execute a certain action type -- attempt to open the door with the key -- but she is uncertain in which action token the execution will result: if she sees to it that the door will be opened or not. 

In order to formalize that idea, BT+AC model is extended with the set of  indistinguishability relations $ \{ \sim_i \}_{i \in Ags}$, where every such relation  is defined on the set on indices. The idea behind this component is classical for epistemic modal logic: an agent at an index knows that a formula is true iff the formula holds in all indices indistinguishable with the current one for that agent. 

Three components should be added to BT+AC model in order to illustrate action types and their connection with action tokens. The finite set of primitive action types is $Type = \{ t_1, t_2, \ldots, t_n \}$. Two functions connecting action types to action tokens are defined. The \textit{execution function} $[\: ] : Ags \times Type \times  Tree \rightarrow 2^{Tree \times H}$ takes an agent $i$, a moment $m$ and an action type $t$ and returns a specific action token $[t]^m_i \in Choice^m_i$, which corresponds to the set of outcomes of executing $t$ by $i$ at $m$. For the sake of simplicity, we write $[t]^m_i$ instead of $[\:](i, t, m)$.

The reverse function, $Label: Ags \times  2^{Tree \times H} \rightarrow Type$ takes an agent $i$ and an action token $X \in Choice^m_i$ and returns the corresponding action type of $X$. Both functions are partial: $[ \: ]$ should be partial since not every action type is available for an agent in any context and $Label$ should be partial as well since not every subset of indices is an action token for any agent. 

Two natural constraints connecting the two functions are:

\begin{enumerate}
    \item if $X \in Choice^m_i$, then $[Label(i, X)]^m_i = X$
    \item if $[t]^m_i$ is defined, then $Label(i, [t]^m_i) = t$
\end{enumerate}

Keeping that notions in mind, we can finally define the syntax of the kstit logic and its semantics.


\begin{definition}[$\mathcal{L}_{kstit}$ syntax]
The language of $\mathcal{L}_{kstit}$ is:
 
 \[
\phi : = p \: | \: \neg \phi \: | \: \phi \lor \phi \: | [stit]_i \phi \: | \: [kstit]_i \phi \: | \: \Box \phi \: | \: K_i \phi
\]

\noindent where $p \in Var, i \in Ags$.
 
 \end{definition}

\begin{definition}[Labeled stit model]


\[
M =  \langle Tree, < , Choice, Ags,  \{ \sim_i \}_{i \in Ags}, Type, [ \: ], Label, \nu \rangle 
\]

\end{definition}
\begin{definition}[$\mathcal{L}_{kstit}$ semantics]


\noindent $\mathcal{M}, m/h \models p \Leftrightarrow p \in \nu (p)$\\
$\mathcal{M}, m/h \models \neg \phi \Leftrightarrow \mathcal{M}, m/h \not\models \phi$\\
$\mathcal{M}, m/h \models \phi \lor \psi \Leftrightarrow \mathcal{M}, m/h \models \phi \mbox { or } \mathcal{M}, m/h \models \psi$\\
$\mathcal{M}, m/h \models \Box \phi \Leftrightarrow \forall h' \in H_m (\mathcal{M}, m/h' \models \phi)$\\
$\mathcal{M}, m/h \models [stit]_i\phi \Leftrightarrow \forall h' \in Choice^m_i (h) (\mathcal{M}, m/h' \models \phi)$\\
$\mathcal{M}, m/h \models K_i \phi \Leftrightarrow \forall m'/h' (m/h \sim_i m'/h' \rightarrow \mathcal{M}, m'/h' \models \phi)$\\
$\mathcal{M}, m/h \models [kstit]_i \phi \Leftrightarrow \forall m'/h' \big( m/h \sim_i m'/h' \rightarrow \\  (Label (i, Choice^m_i(h)) = Label (i, Choice^{m'}_i(h')) \land \mathcal{M}, m'/h' \models \phi )\big)$

\end{definition}

Horty and Pacuit suggest two basic constraints on the interplay between action types and agents' knowledge. Tt is easy to see that the second one is  derivable from the first one:
\begin{enumerate}
    \item If $m/h \sim_i m'/h'$, then $Label(i, Choice^m_i(h)) = Label(i, Choice^{m'}_{i}(h'))$
    \item  If $m/h \sim_i m'/h'$, then $[Label(i, Choice^m_i(h))]^{m'}_i$ is defined
\end{enumerate}

Informally speaking, (1) says that agent knows what action types she executes: if two indices are indistinguishable for some agent, then the agent executes actions of the same type in both indices. From this statement it follows that (2) -- the same action types should be available for the agent in all indices, indistinguishable for her.
